ActiveClean: Interactive Data Cleaning While Learning Convex Loss Models

Data cleaning is often an important step to ensure that predictive models, such as regression and classification, are not affected by systematic errors such as inconsistent, out-of-date, or outlier data. Identifying dirty data is often a manual and iterative process, and can be challenging on large datasets. However, many data cleaning workflows can introduce subtle biases into the training processes due to violation of independence assumptions. We propose ActiveClean, a progressive cleaning approach where the model is updated incrementally instead of re-training and can guarantee accuracy on partially cleaned data. ActiveClean supports a popular class of models called convex loss models (e.g., linear regression and SVMs). ActiveClean also leverages the structure of a user's model to prioritize cleaning those records likely to affect the results. We evaluate ActiveClean on five real-world datasets UCI Adult, UCI EEG, MNIST, Dollars For Docs, and WorldBank with both real and synthetic errors. Our results suggest that our proposed optimizations can improve model accuracy by up-to 2.5x for the same amount of data cleaned. Furthermore for a fixed cleaning budget and on all real dirty datasets, ActiveClean returns more accurate models than uniform sampling and Active Learning.

==> algorithm.tex <==
\section{Model Processing}

\subsection{Error Predicate Case} 
For a tuple $(x_j,y_j)$, there are basically two cases:
\[
(x_j,y_j)= \begin{cases} (x_j,y_j) &\rho_i \text{ is false} \\ 
(C_i(x_j),C_i(y_j)) & \rho_i \text{ is true} 
\end{cases} 
\]
We can calculate the average change over already cleaned data that satisfy the predicate\footnote{For added features, we create dummy feature vectors in the dirty data}:
\[
\Delta_i = \sum_{j \in \rho(cleaned)} (C_i(x_j),C_i(y_j)) - (x_j,y_j)
\]
the resulting estimator is:
\[
\hat{C}_i= \begin{cases} (x_j,y_j) &\rho_i \text{ is false} \\ 
(x_j,y_j) + \Delta_i & \rho_i \text{ is true} 
\end{cases} 
\]

The oracular algorithm gets modified as follows:
\begin{enumerate}[noitemsep]
\item Initialize all $\Delta = 0$
\item For rounds i=1...T
\begin{enumerate}
	\item For each cleaning op j=1...K
	\begin{enumerate}
		\item For all points that do not satisfy $\rho_j$, calculate the average gradient and call this result $g_1$.
		\item For all points that do satisfy $\rho_j$, sample $\frac{B}{T}$ data points using $\hat{C}_j$ described above.
		\item Apply data cleaning to the sample of data, or if already cleaned skip.
		\item For all newly cleaned points update $\Delta_j$
		\item Calculate weighted gradient of the sample points call this $g_2$.
		\item For $N_1$ points that do not satisfy the predicate and $N_2$ points that do,  apply gradient descent using the gradient $\frac{N_1g_1 + N_2g_2}{N_1 + N_2}$.
	\end{enumerate}
\end{enumerate}
\item Return $\theta^{(T)}$
\end{enumerate} 

To actually implement this algorithm efficiently there are physical design considerations that we will discuss in the next section.

\subsubsection{Error Predicate Case: Analysis}
Using the error predicates can significantly increase the accuracy when errors are sparse.
In fact, this saving is quadratic in the sparsity $O(sparsity^2)$.
\begin{theorem}
The error-predicate algorithm converges to the correct answer.
Furthermore, suppose there are $N_1$ erroneous points out of $N$ total points.
\[\sigma^2_{ep} = \frac{N^2_1\sigma^2_{imp}}{N^2}\]
\end{theorem}
\begin{proof}
Gradient is unbiased at each step.
\reminder{Probably cite TR for proof}
\end{proof}

\subsection{General Case}
Finally, in the general case, we do not know the error predicate in advance.
Consider a crowd-based cleaning technique whose effects are hard to predict a priori. 
In this case, we have to continuously update a classifier to partition the data into 
clean and dirty.
The challenge is that this potentially biases our result if our classifier is not perfect.
Some dirty points may be classified as clean.
The quadratic savings seen in the predicate case can often outweigh small biases due to classification error.

Like before, suppose we decomposed the function $C$ into its consituent cleaning operations ${C}_i^{k}$.
For each cleaning operation, we have a classifier, e.g., Support Vector Machine, that learns which points are dirty and which points are cleaned based on that operation.
To account for potential bias in the classifier, we allow the analyst to specify the design point in the bias variance tradeoff.
Many types of classifiers allow users to tradeoff precision and recall.
For an SVM, we may only classify a point as clean if it is sufficiently far from the margin.
Or for Logistic Regression, we may do so if its class likelihood is over 80\%.
In our experiments, we use SVMs and the margin distance provides a flexible way to tradeoff potential bias and gradient variance.

Adding the classifier also adds a complex depedence between batch size and performance.
Initially, the classifier is likely very inaccurate due to the lack of training examples.
As we clean more data, we can learn what is clean and what is dirty.
Accordingly, we can delay the classifier's introduction by $l$ iterations until such time it is accurate. 

\begin{enumerate}[noitemsep]
\item Initialize all $\Delta = 0$
\item For rounds i=1...T
\begin{enumerate}
	\item For each cleaning op j=1...K
	\begin{enumerate}
		\item If $i \ge l$, apply classifier to partition dirty and cleaned data.
		\item Follow error predicate algorithm steps ii-v
		\item For $N_1$ ``clean" points and $N_2$ ``dirty" points, apply gradient descent using the gradient $\frac{N_1g_1 + N_2g_2}{N_1 + N_2}$.
		\item Update classifier with newly cleaned data.
	\end{enumerate}
\end{enumerate}
\item Return $\theta^{(T)}$
\end{enumerate} 

The general case algorithm is harder to analyze and thus we rely on empirical performance on real data.






==> coverletter.tex <==
{\noindent \normalsize \bf Dear SIGMOD Chair and Referees: }

\vspace{.5em}

We thank the reviewers and chair for the helpful feedback on our paper. 
We addressed all of the concerns and included references to the revised text. 
To summarize the major changes:

\begin{enumerate}
\item Sections 1 and 2 clarify the contributions of \sys and its relationship to related work.

\item In Section \ref{dmodel}, we formalize the definition of dirty data and the data cleaning model.

\item Section \ref{s:usecase} presents a running example that is referenced in each technical section (Examples \ref{archex}, \ref{upex},\ref{detex1},\ref{detex2},\ref{estex}).

\item In Section \ref{statements}, we revised the problem statement to be independent of our solution method. The section highlights two subproblems, correctness and efficiency, which are used to organize the technical sections.

\item Section \ref{arch} presents a revised system architecture that first emphasizes the essential components for correctness, and then highlights optional optimizations. 

\item We have re-organized and re-written the technical sections to improve readability (Sections \ref{model-update}-\ref{opti}).

\item We include references to all of the related work suggested by the reviewing committee \cite{whang2014incremental, papenbrock2015progressive, gruenheid2014incremental, DBLP:journals/pvldb/YakoutENOI11, yakout2013don, heise2014estimating}.
\end{enumerate}


\subsection*{Overview} 
Data cleaning is often applied before featurization and predictive modeling to provide clean training data.
Corruption of the training data can degrade model quality, and high-dimensional models can amplify small errors.
Unfortunately, data cleaning is often a manual and time consuming process, and may be impractical for very large datasets.
\sys is a framework that allows users to train accurate models without having to clean the entire dataset. 
\sys couples data cleaning with model training to leverage information from the model to identify records that maximally improve accuracy.
The paper shows that naive integration of data cleaning and model training can lead to convergence problems, and we present a novel framework for training on partially clean data.
Specifically, it applies: (1) a gradient-based update derived from small batches of cleaned data, (2) weighted sampling to carefully select these batches, (3) optimizations to select records that are most likely to be dirty.

As the name implies, \sys is inspired by active learning and both seek to improve the efficiency of expensive manual or crowdsourced data cleaning.
Prior work applies active learning to most efficiently clean an entire dataset--independent of the user's desired analysis after data cleaning.
In contrast, for a large class of predictive models, \sys prioritizes data cleaning by identifying records, which if cleaned, are likely to change the model's predictions.
The key new challenge is that model training on a mixture of clean data and not-yet-cleaned dirty data, can lead to severe inaccuracy due to a well-studied phenomenon called Simpson's paradox (Section \ref{correctness}).
Consequently, we propose a new model update algorithm that provably avoids this problem, and integrate the prioritization with this algorithm.

\vspace{0.5em}

\subsection*{Meta Review Details} 

\noindent\noindent \textbf{M1. There should be a formal vocabulary introduced early on. The exact idea of ``dirty" here can be hard to follow: what is the exact error type(s) that the system is intended to clean?}

\vspace{0.5em}

We added a section that clarifies that our system supports data cleaning operations that can be represented as record-by-record mappings (Section \ref{dmodel}).
Formally, there exists a function (implemented via human or algorithm) that given a dirty record will return a unique clean record.
This definition does not include errors that simultaneously affect multiple records such as duplication or schema transformation problems.
We emphasize this limitation early in the introduction (Section 1) and background (Section 2)sections.

%Details are provided in Response \textbf{R2.1}.

\vspace{0.5em}

\noindent\textbf{M2a. Sections 5-7 are the technical core of the paper, and appear formal at the expense of aiding understanding.}

We have revised the technical sections of the paper to improve readability by moving derivations to the appendix and including three new examples.

\vspace{0.5em}

\noindent \textbf{M2b. They appear to implement something that resembles active learning or bootstrapping, except inside the gradient descent loop. The motivation of some of this is not clear; is it necessary to integrate with the gradient descent?} 

Yes, the integration with gradient descent is necessary as it allows for provable guarantees about the model's convergence.
We have revised the paper to intuitively motivate this problem in Section \ref{correctness}, formally describe the problem in Section \ref{updp}, and simplified the presentation of the gradient-based update solution in Section \ref{geod}.

\vspace{0.5em}

\noindent\textbf{M2c. This is not how most active learning methods are implemented. Is it possible to implement these approaches in a way that is orthogonal to the SGD algorithm? The current writeup entangles some of these design choices.} 

We have revised the paper to decouple two subproblems: (1) the correctness problem of how to update a model after cleaning, and (2) the efficiency problem of how to prioritize cleaning using the model. 
Problem (1) is addressed with SGD.
The solution to problem (2) is independent of the update problem, although we highlight its optimality properties with respect to SGD.
We clarify that any sampling algorithm that ensures that all dirty records have a non-zero sampling probability can be applied.
We also have re-organized the paper to isolate optimizations from the essential components of \sys.
In the revision, Section \ref{opti} describes optimizations that improve the convergence rate of the system.
%We describe a number of cases when these optimizations are possible.

\vspace{0.5em}

\noindent\textbf{M3. In general, the distinction between an ``architecture" and an ``algorithm that fits into the architecture" is quite unclear. The problem with SGD/Active Learning above is one example.}

We have significantly revised the architecture section of the paper.
We first separate the formal problem statement (Section \ref{statements}) and system architecture (Section \ref{arch}).
The architecture section now describes the essential data flows of the system and is orthogonal to the solutions of the problems described in Section \ref{statements}.
We also differentiate the essential components of the architecture and the optional instance-specific optimizations.
The new architecture would apply even if the model update problem was addressed with a different algorithm (i.e., not SGD).
%We also clearly identify the user inputs in Section \ref{uinp}.

\vspace{0.5em}

\noindent\textbf{M4. The paper, and especially the technical sections, would benefit enormously from a detailed running example showing how the algorithm works}

We have added examples to each of the technical sections based on our running example of an analyst using an SVM for fraud detection. 
Section 4 (Architecture) describes an intuitive end-to-end application (Example \ref{archex}).
Section 5 (Update Problem) describes how updates are propagated and calculated (Example \ref{upex}).
%Section 7.1 (Detection) contains two examples for how the two different types of detectors can be used (Examples \ref{detex1} and \ref{detex2}).
Section 7.2 describes how to apply the optimizations to this example.

\vspace{0.5em}

\noindent\textbf{M5. Some connections to related work that combines machine learning and data cleaning should be made. See the other reviewers' comments.}

We have added Section \ref{alrw} to connect \sys to related work that applies machine learning to data cleaning.
This was a source of significant confusion in the initial submission, and we have clarified the key differences.
We have also revised our related work section to highlight the suggested references to progressive data cleaning and entity resolution~(Section \ref{rw}).
%Details are provided in Response \textbf{R1.4} and Response \textbf{R2.2}.

\subsection*{Review 1 Details} 

\noindent\textbf{R1.1: At first, the problem seems a bit too specialized. The abstract is too loaded with technical terms and a turn-off. This is then mitigated in the introduction. \\
As mentioned above, the abstract is (to me) overly technical and did not make me curious. I did not know off the bat what a convex loss model is, what importance sampling is, etc.}

\noindent We revised the abstract to better motivate our problem and solutions:

\emph{Data cleaning is often applied before predictive modeling, such as regression and classification, to provide clean training data.
The high dimensionality of predictive models can amplify small amounts of data error leading to error-prone predictions.
Unfortunately, data cleaning can be a manual and time consuming process, and may be impractical for very large datasets.
This paper explores techniques to train accurate models without having to clean the entire dataset.
We propose \sys, a progressive cleaning approach where data is simultaneously cleaned as the model is trained.
As more data is cleaned, the accuracy of the model gradually converges.
The challenge is that models trained on partially cleaned data can be arbitrarily incorrect; requiring a new algorithm for incrementally updating results given newly cleaned data.
\sys supports a popular class of models called convex loss models (e.g., linear regression and SVMs) and record-by-record data cleaning operations.
By coupling data cleaning and model training, \sys can leverage the structure of a user's model to prioritize cleaning those records likely to affect the results.
Evaluation on four real-world datasets suggests that for a fixed cleaning budget, \sys returns more accurate models than uniform sampling and Active Learning when corruption is systematic and sparse. }

\vspace{0.5em}

\noindent\textbf{R1.2: Poor embrace of the duplicate detection problem (see details below). Your model of the cleaner seems to preclude any duplicate detection, which certainly cannot happen on individual records. Also you extension for a set of record does not fit the problem of duplicate detection. This is in contrast, for instance, to your ER example in the second column of that page. Appendix A.1 is misleading here, as you mention with Example 7 ``in entity resolution problems..." but do not actually address that problem in the example. Fixing some common inconsistency is not entity resolution.}

We apologize for the confusing terminology and have revised our paper to clarify that we do not address record-level deduplication and entity resolution.

\vspace{0.5em}

\noindent\textbf{R1.3: Cheated by using a narrower font than required. Will have trouble with camera ready copy if publisher insists on proper font.\\
- I would not use ``overview" as a verb...
- 3.2: the detector select -> the detector selects
- 4.3: Wrong quotation marks around ``learning".
- QED symbols on page 8 are ugly when placed directly after formula. 
- References need a clean up. Just as an example: Venue is missing for [24], year is mentioned 3 times for [8], [11], etc. Page numbers appear sporadically.}

\noindent We have addressed all of the formatting and copy editing issues.

\vspace{0.5em}

\noindent\textbf{R1.4:There is some related work specifically addressing progressive/incremental entity resolution. You might want to point your readers to this.
\\E.g.
\\- Incremental entity resolution on rules and data, Whang et al. VLDB Journal 2014
\\- Progressive duplicate detection, Papenbrock et al., TKDE 2015
\\- Incremental record linkage, Gruenheid et al., PVLDB 2014
\\- Another work that is related is ``Estimating the Number and Sizes of Fuzzy-Duplicate Clusters" by Heise et al. CIKM 2014, which also incrementally cleans samples of data to predict in this case the number of record matches.}

Thank you for highlighting these references, and we have included them in our related work:

\emph{When data cleaning is expensive, it is desirable to apply it \textbf{progressively}, where analysts can inspect early results with only $k \ll N$ records cleaned.
Progressive data cleaning is a well studied problem especially in the context of entity resolution \cite{altowim2014progressive, whang2014incremental, papenbrock2015progressive, gruenheid2014incremental}.
Prior work has focused on the problem of designing data structures and algorithms to apply data cleaning progressively. which is challenging because many data cleaning algorithms require information from the entire relation.
Over the last 5 years a number of new results have expanded the scope and practicality of progressive data cleaning~\cite{mayfield2010eracer, DBLP:journals/pvldb/YakoutENOI11, yakout2013don}.
\sys studies the problem of prioritizing progressive cleaning by leveraging information about a user's subsequent use for the data.
Certain records, if cleaned, may be more likely to affect the downstream analysis.\\
SampleClean~\cite{wang1999sample} applies data cleaning to a sample of data, and estimates the results of aggregate queries.
Sampling has also been applied to estimate the number of duplicates in a relation \cite{heise2014estimating}. 
Similarly, Bergman et al. explore the problem of query-oriented data cleaning \cite{DBLP:conf/sigmod/BergmanMNT15}, where given a query, they clean data relevant to that query. 
Existing work does not explore cleaning driven by the downstream machine learning ``queries" studied in this work.}

\vspace{0.5em}

\noindent\textbf{- Page 1, last paragraph in column 1 reads as if reference to [3] is a reaction to the work referenced in the previous sentence, i.e., the term ``remains" is misleading.
- I did not quite understand the short paragraph on crowd-sourcing. Why is this even relevant?
 I believe it would suffice to simply state that cleansing is expensive...}

We appreciate the thorough feedback and have tightened up the writing in the introduction. In particular, we have consolidated the motivation to a single paragraph describing the expense of data cleaning. We include a single sentence referencing related work on crowdsourcing/human-guided data cleaning.


\subsection*{Review 2 Details}

\noindent\textbf{R2.1: The definition of ``clean data" is imprecise and not clear. It appears that ``cleaning" in this system refers to entity resolution, cleaning w.r.t. dependencies, and possibly other actions as needed by the application. This makes it difficult to gauge overall accuracy when there are different interpretations of cleanliness. It is not clear how entity resolution and cleaning w.r.t. dependencies can be done holistically.}

We added Section \ref{dmodel} to the paper which clarifies the supported data cleaning operations:

\emph{\sys supports data cleaning operations that can be represented as record-by-record transformations.
Formally, there exists a function (implemented via human or algorithm) that given a dirty record will return a unique clean record.
This definition does not cover errors that simultaneously affect multiple records such as record duplication or schema transformation problems.
We represent this operation as $C(\cdot)$ which can be applied to a record $r$ to recover the clean record $r' = C(r)$.
Therefore, for every $r \in R$ there exists a unique $r' \in R^*$, where $R^*$ is the hypothetical fully cleaned relation.
We assume that there is a featurizer $F(\cdot)$ that maps a record to a feature vector $x$ and a label vector $y$.
So each record corresponds to one training example for the downstream model.}

\vspace{0.5em}

Our appendix (Section \ref{set-of-r}) also describes an extension to this model where sets of records can be cleaned at once (e.g., a find-and-replace operation).

\vspace{0.5em}

\noindent\textbf{R2.2: The paper describes a problem setting focused on modelling the iterative cleaning process rather than actual data management problems. The paper may be better suited at an ML venue.}

Over the last 5 years a number of new results have expanded the scope of progressive and interactive data cleaning~\cite{mayfield2010eracer, DBLP:journals/pvldb/YakoutENOI11, yakout2013don, altowim2014progressive, whang2014incremental, papenbrock2015progressive, gruenheid2014incremental}.
However,  it turns out that the straight-forward integration of existing progressive data cleaning methods with model training can lead to error-prone and misleading results due to the well studied Simpson's paradox (Section \ref{correctness}).
Recognizing that data analytics is increasingly moving towards predictive modeling, \sys presents an initial exploration of this problem.  

\vspace{0.5em}

\noindent\textbf{R2.3: Missing references to related work on interactive data cleaning. For the comparative evaluation, 2/3 techniques are ML based techniques, not interactive data cleaning systems. See D2.\\
D2: Data cleaning systems have also considered interactive engagement with the user and the application of ML techniques. 
i) Mohamed Yakout, Laure Berti-Equille, Ahmed K. Elmagarmid. Don't be SCAREd: use SCalable Automatic REpairing with maximal likelihood and bounded changes. SIGMOD Conference 2013: 553-564
ii) Mohamed Yakout, Ahmed K. Elmagarmid, Jennifer Neville, Mourad Ouzzani, Ihab F. Ilyas.
Guided data repair. PVLDB 4(5): 279-289 (2011).
}

Prior work in data cleaning applies active learning to most efficiently clean an entire dataset--independent of the user's desired analysis after data cleaning.
On the other hand, \sys explores the problem of data cleaning to provide clean training data for a predictive modeling problem.
It identifies records to clean that maximally change the user's modeling results.
We added Section \ref{alrw} to clarify this distinction:

\emph{Next, we contrast \sys and existing data cleaning approaches.
Machine learning, specifically active learning, has been applied in prior work to improve the efficiency of data cleaning~\cite{yakout2013don,DBLP:journals/pvldb/YakoutENOI11,gokhale2014corleone}.
Human input, either for cleaning or validation of automated cleaning, is often expensive and impractical for large datasets.
A model can learn rules from a small set of examples cleaned (or validated) by a human, and active learning is a technique to carefully select the set of examples to learn the most accurate model.
This model can be used to extrapolate repairs to not-yet-cleaned data, and the goal of these approaches is to provide the cleanest possible dataset--independent of the subsequent analytics or query processing.\\
As the name implies, \sys is inspired from active learning as both seek to improve the efficiency of expensive data cleaning.
In contrast, \sys addresses a very different problem, namely, how information about a user's subsequent data analysis can inform which data to clean.
If the cleaned data will ultimately be used as training data in a predictive model, \sys presents an algorithm to prioritize those data that are most likely to change the result.
The key new challenge is correctness.
Models trained on partially clean data can have severe inaccuracies.
Thus, existing approaches, which are designed for homogeneous data, cannot be applied.
One of the primary contributions of this work is an incremental model update algorithm with correctness guarantees for mixtures of data.
An active learning-like algorithm can be applied in conjunction with the proposed model update algorithm while preserving correctness.
However, the new problem setting also has several additional opportunities for optimizations, which empirically can significantly improve the convergence rate of typical active learning criteria (Section \ref{eval}).}

\vspace{0.5em}

We also included additional details in the related work section (Section \ref{rw}):

\emph{There are a number of other works that use machine learning to improve the efficiency and/or reliability of data cleaning~\cite{DBLP:journals/pvldb/YakoutENOI11,yakout2013don,gokhale2014corleone}.
For example, Yakout et al. train a model that evaluates the likelihood of a proposed replacement value \cite{yakout2013don}.
Another application of machine learning is value imputation, where a missing value is predicted based on those records without missing values.
Machine learning is also increasingly applied to make automated repairs more reliable with human validation \cite{DBLP:journals/pvldb/YakoutENOI11}.
Human input is often expensive and impractical to apply to entire large datasets.
Machine learning can extrapolate rules from a small set of examples cleaned by a human (or humans) to uncleaned data \cite{gokhale2014corleone, DBLP:journals/pvldb/YakoutENOI11}.
This approach can be coupled with active learning \cite{DBLP:journals/pvldb/MozafariSFJM14} to learn an accurate model with the fewest possible number of examples.
While, in spirit, \sys is similar to these approaches, it addresses a very different problem of data cleaning before user-specified modeling.
The key new challenge in this problem is ensuring the correctness of the user's model after partial data cleaning.}

\textbf{R2.4: Sampling is an important part of the framework and influences the accuracy of the cleaning. Yet, there is little discussion on sampling rate, or how a sample is chosen.}

We have added a new section (Section 6), which is dedicated to describing the basic sampling algorithm.
Section 7 has been revised to describe optimizations to this algorithm.

\vspace{0.5em}

\textbf{R2.5: An end-to-end running example in Section 5 is needed to highlight the intuition of the cleaning process.}

We included a running example of fraud detection on dirty data. Each of the technical sections ends with a reference to this running example (see response \textbf{M4}).


\vspace{0.5em}


\subsection*{Review 3 Details}
\noindent\textbf{R3.1: The authors do not distinguish between the system architecture and the individual issues that they are presenting.}

Response \textbf{M3} describes several revisions to the architecture including: separating problem formalization and architecture, discussing the data flow rather than the algorithms, and differentiating the essential components for correctness from optimizations.

\vspace{0.5em}

\noindent\textbf{R3.2: The paper uses lots of definitions, and a multitude of that do not necessarily contribute to readability.
Without being an expert in the field, I found it extremely difficult to follow the paper as it touches upon multiple problems at the same time: data cleaning, model training, convex analytics, etc., uses definitions, notation and lots of examples that did not allow me to have a global understanding of the work.\\
I would prefer to have a more focused paper on one of these aspects that has concrete goals and then, having an overview of the architecture of the system as a small section. I believe that the architecture should not be the focus and the skeleton of this paper. Instead, I believe that the authors could focus on the individual problems.}

We have discussed a number of specific textual revisions in response \textbf{M2} and \textbf{M3}. Here are a list of other revisions to improve the readability:

\begin{enumerate}
\item We have significantly revised the paper to make it more accessible and readable. Where possible, we have simplified, or even removed, notation and definitions. We also included Section \ref{notation} to summarize all of the important notation before the technical sections.
\item We have expanded the background section to provide a more detailed setup and context to the problem.
\item We revised the technical sections to first present a minimum viable solution that addresses the two subproblems (Section \ref{model-update} and Section  \ref{dist-samp}).
\item The next section (Section \ref{opti}) describes optional optimizations that can be applied in a number of practical cases.
\item Detailed derivations are now in the appendix, and the additional space has been used for three new examples in the technical sections (Sections \ref{model-update}-\ref{opti}).
\end{enumerate}


==> detect.tex <==
\section{Partitioning Data With Detection}\label{det}
\sys can improves the progress of each update iteration by intelligently partitioning the data into expected dirty and clean partitions. 
This ensures that the sampler draws data that are likely to be dirty.

\subsection{Goals}
The detector returns two important aspects of a record: (1) whether the record is dirty, and (2) if it is dirty, what is wrong with the record.
The sampler can use (1) to select a subset of dirty records to sample at each batch. 
The estimator can use (2) estimate the value of data cleaning based on other records with the same corruption.
\sys supports two types of detectors: \emph{a priori} and \emph{adaptive}.
In the \emph{a priori} case, there is a way to select the set of dirty records before any cleaning.
This case is possible for some types of data errors.
In the adaptive case, detection is learned as data is cleaned.

\subsection{\protect\textit{\large A Priori} Case}
For many types of dirtiness such as missing attribute values and constraint violations, it is possible to efficiently enumerate a set of corrupted records and determine how the records are corrupted.

\begin{definition}[A Priori Detection]
Let $r$ be a record in $R$. An a priori detector is a detector that returns a Boolean of whether the record is dirty and a set of columns $e_r$ that are dirty.
\[
D(r) = (\{0,1\}, e_r)
\]
From the set of columns that are dirty, find the corresponding features that are dirty $f_r$ and labels that are dirty $l_r$.
\end{definition}

\noindent Here are example use cases of this definition using data cleaning methodologies proposed in the literature.

\vspace{0.5em}

\noindent\textbf{Constraint-based Repair: }
One model for detecting errors involves declaring constraints on the database.

\vspace{0.5em}

\emph{Detection. } Let $\Sigma$ be a set of constraints on the relation $\mathcal{R}$. 
In the detection step, the detector selects a subset of records $\mathcal{R}_{dirty} \subseteq \mathcal{R}$ that violate at least one constraint.
The set $e_r$ is the set of columns for each record which have a constraint violation. 

\begin{example}\label{detex1}
An example of a constraint on the running example dataset is that the \texttt{status} of
a contribution can be only ``allowed" or ``disallowed".
Any other value for \texttt{status} is an error.
\end{example}

\subsection{Adaptive Detection}
\emph{A priori} detection is not possible in all cases.
The detector also supports adaptive detection where detection is learned from previously cleaned data.
Note that this ``learning" is distinct from the ``learning" at the end of the pipeline.
The challenge in formulating this problem is that detector needs to describe how the data is dirty (e.g. $e_r$ in the \emph{a priori} case).
The detector categorizes the corruption into $u$ classes.
These classes are corruption categories that do not necessarily align with features, but every record is classified with at most one category.

When using adaptive detection, the repair step has to clean the data and report to which of the $u$ classes the corrupted record belongs.
When an example $(x,y)$ is cleaned, the repair step labels it with one of the ${\text{clean}, 1,2,...,u+1}$ classes (including one for ``not dirty").
It is possible that $u$ increases each iteration as more types of dirtiness are discovered. 
Then, the detection problem reduces to a multiclass classification problem.
This problem can be addressed by any multiclass classifier, and we use an all-versus-one SVM in our experiments.

\begin{definition}[Adaptive Case]
Select the set of records for which $\kappa$ gives a positive error classification (i.e., one of the $u$ error classes).
After each sample of data is cleaned, the classifier $\kappa$ is retrained.
So the result is:
\[D(r) = (\{1,0\},\{1,...,u+1\})\]
\end{definition}

\vspace{0.75em}

\noindent\textbf{Adaptive Detection With OpenRefine: }
\begin{example}\label{detex2}
OpenRefine is a spreadsheet-based tool that allows users to explore and transform data.
However, it is limited to cleaning data that can fit in memory on a single computer.
Since the cleaning operations are coupled with data exploration, \sys does not know what is dirty in advance (the analyst may discover new errors as she cleans).

Suppose the analyst wants to use OpenRefine to clean the running example dataset with \sys.
She takes a sample of data from the entire dataset and uses the tool to discover errors.
For example, she finds that some drugs are incorrectly classified as both drugs and devices.
She then removes the device attribute for all records that have the drug name in question.
As she fixes the records, she tags each one with a category tag of which corruption it belongs to.
\end{example}

==> impestimate <==
\section{Approximating the Optimal Distribution}
We do not know what the clean value of the gradient is so we have to estimate this clean value.
We want to derive our estimate in such a way that we can decouple the different cleaners.
For each cleaner $i$, we should be able to estimate a $\Delta_i$ which is an expected incremental effect of the cleaner.
In this section, we formalize this problem with a first order approximation of the expected gradient.

The expected gradient is defined as:
\[
\mathbb{E}(\nabla\phi(x_{clean},y_{clean},\theta^{(t)}))
\]
Since, we do not know this value, we can take the expected value of the Taylor series expansion around the dirty value.
Let us first consider the case where a single column is updated. 
There are two cases: (1) either a feature $X$ is updated or an obersvation $Y$ is updated.

\noindent \textbf{Feature Cleaned: } 
\[
\nabla\phi(x,y,\theta^{(t)}) + \frac{\partial}{\partial X}\nabla\phi(x,y,\theta^{(t)})\cdot \mathbb{E}(\Delta x)+...~~\blacksquare
\]

\noindent \textbf{Observation Cleaned: } 
\[
\nabla\phi(x,y,\theta^{(t)}) + \frac{\partial}{\partial Y}\nabla\phi(x,y,\theta^{(t)})\cdot \mathbb{E}(\Delta y)+...~~\blacksquare
\]

The linearity of the Taylor series expansion allows us to sum up the $\Delta$ changes for each column.
\begin{lemma}[Additive Changes]
For changes to all columns, the Taylor Series expansion is:
\[\nabla\phi(x,y,\theta^{(t)}) + \sum_i \frac{\partial}{\partial X_i}\nabla\phi(x,y,\theta^{(t)})\cdot \mathbb{E}(\Delta_i x) \]
\[+ \sum_j \frac{\partial}{\partial Y_j}\nabla\phi(x,y,\theta^{(t)})\cdot \mathbb{E}(\Delta_j y)\]
\end{lemma}
\noindent Since cleaners operate on disjoint attributes:
\begin{theorem}[Cleaner Decoupling]
For a set of cleaners $C_{1} \circ C_{2} \circ ... C_{k}$, we can associate a vector $\bar{\Delta}_i$ which is equal to:
\[
\bar{\Delta}_i = \sum_i \frac{\partial}{\partial X_i}\nabla\phi(x,y,\theta^{(t)})\cdot \mathbb{E}(\Delta_i x)
\]
\end{theorem}

\subsection{Approximation Quality}
Next, we explore the quality of this approximation.
The error in the Taylor series is given by the higher derivatives:
\[
+ \frac{1}{2}\frac{\partial^2}{\partial X_i}\nabla\phi(x,y,\theta^{(t)}\cdot \mathbb{E}(\Delta_i x^2) + \frac{1}{6}\frac{\partial^3}{\partial X_i}\nabla\phi(x,y,\theta^{(t)}\cdot \mathbb{E}(\Delta_i x^3) + ...
\]
For many common loss functions, these higher derivatives are zero.


\subsection{Relative Benefit}

We analyze the conditions under which this estimate results in a more accurate 




\subsection{Putting it into practice}
Part of the motivation of this work is that the function $\mathcal{D}$ is often expensive to evaluate.
Instead, suppose we had an estimate of $\hat{\mathcal{D}}$ that was cheap to evaluate.
We could then apply this estimate to every point and get an approximately optimal sampling distribution.
This builds the inutition for the basic algorithm that we will propose.
As we clean data, we learn an estimator $\hat{C}$ which can be used to calculate the approximately optimal sampling distribution.




==> optimizer.tex <==
\section{Adaptive Error Detection}\label{imperfect} 
In this section, we explore how we can handle the case where the error detection is learned as we clean data.

\subsection{Challenges}
In this section, we explore the partitioning model, where as we clean more data, we iteratively prune data we expect to be clean from $R_{dirty}$.
This is done with a classifier that is updated with new training data based on the previous iterations results.
The main challenge is that the sampling weights calculated in the previous section are dependent on the error detection step returning a set of corrupted features.
When we relax this assumption, there are new challenges in error estimation.
Next, an important aspect of our gradient update is partitioning the dirty and clean data.
We aggregate an average gradient from both subpopulations when making our update.
However, in some cases, characterizing this partioning can be difficult and it may be impossible to ensure this condition unless $R_{dirty} = R$ causing a loss in efficiency if errors are sparse. 

\subsection{Error Classes}
When we relax the restrictions on the error detection step, we no long have a set of corrupted features $e_r$.
This breaks the decoupling argument that we made in the previous section.
However, our high-level goal in the previous section, was to estimate the gradient for groups of similarly corrupted records.
We try to formulate an analogous methodology that generalizes what we did in the previous section to error detection steps that are learned over time.
Instead of assuming that we know which features are corrupted, let us say that we know that there are $u$ classes of errors.
As the analyst cleans data, she tags dirty data with one of the $u$ classes.
Then, the error detection problem reduces to a multiclass classification problem.
Once classified, we can apply an average change conditioned on the error class.

With this intuition in mind, we have to revise our error repair step:
\vspace{0.5em}

\noindent\textbf{Error Repair: } When an example $(x,y)$ is cleaned, the repair step also has to provide a label of to which of the ${\text{clean}, 1,2,...,u}$ classes it belongs. It is possible that $u$ increases each iteration as more errors are discovered. 

\vspace{0.5em}

Suppose, we have a multi-class classifier $\kappa$ (e.g. SVM) that classifies every record $r$ into $u+1$ classes (the $u$ error types or not dirty).
Thus, we revise the partitioning in the following way:

\vspace{0.5em}

\noindent\textbf{Error Detection: } To select $R_{dirty}$, we select the set of records for which $\kappa$ give a positive error classification (i.e., one of the $u$ error classes).
Many types of classifiers allow users to tradeoff precision and recall.
In other words, we can also select any record within some level of confidence of the classification margin.
For an SVM, we may only classify a point as clean if it is sufficiently far from the margin.
Or for Logistic Regression, we may do so if its class likelihood is over 80\%.

\subsection{Error Estimate}
Our model update framework still holds in this setting, however, our error estimation framework requires some modification.
In our derivation, we showed that our error estimate was a linearization of the conditional expectation of the gradient.
Instead of conditioning on the features that are corrupted, we condition the error classes.
So for each error class, we compute a $\Delta_{xu}$ and $\Delta_{yu}$.
These are the average change in the features given that class and the average change in labels given that class respectively.
\[
p_{r,u}\propto\|\nabla\phi(x,y,\theta^{(t)}) + M_x \cdot \Delta_{ux} +  M_y \cdot \Delta_{uy}\|
\] 


